Location-based Radiology Report-Guided Semi-supervised Learning for Prostate Cancer Detection

Prostate cancer is one of the most prevalent malignancies in the world. While deep learning has potential to further improve computer-aided prostate cancer detection on MRI, its efficacy hinges on the exhaustive curation of manually annotated images. We propose a novel methodology of semisupervised learning (SSL) guided by automatically extracted clinical information, specifically the lesion locations in radiology reports, allowing for use of unannotated images to reduce the annotation burden. By leveraging lesion locations, we refined pseudo labels, which were then used to train our location-based SSL model. We show that our SSL method can improve prostate lesion detection by utilizing unannotated images, with more substantial impacts being observed when larger proportions of unannotated images are used.

==> figureNsigVsLoc.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.23 \textwidth}
\centering
%\includegraphics[height=1.25in]{PICAI_0025_prob_legend_seg_ax_slice11}
\includegraphics[height=1.25in]{PICAI_0025_prob_legend_seg_ax_slice11.png}
\caption{Probability map}
\end{subfigure}
\begin{subfigure}[t]{0.23 \textwidth}
\centering
\includegraphics[height=1.25in]{PICAI_0025_nsig_seg_ax_slice11.png}
\caption{Lesion count}
\end{subfigure}
\begin{subfigure}[t]{0.23 \textwidth}
\centering
\includegraphics[height=1.25in]{PICAI_0025_les_loc_seg_ax_slice11.png}
\caption{Lesion location}
\end{subfigure}
\begin{subfigure}[t]{0.23 \textwidth}
\centering
\includegraphics[height=1.25in]{PICAI_0025_gt_seg_ax_slice11.png}
\caption{Radiologist}
\end{subfigure}
\caption{All segmentations were overlayed on the T2W image of the MRI. (a) Example cancer probability heatmap for a case with over}
\label{fig:pseudoMaskCountvsLoc}
\end{figure}



==> figureNsigVsLocInference.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.46 \textwidth}
\centering
\includegraphics[height=1.0in]{PICAI_0470_t2w_ax_slice14.png}
\includegraphics[height=1.0in]{PICAI_0470_adc_ax_slice14.png}
\includegraphics[height=1.0in]{PICAI_0470_hbv_ax_slice14.png}
\caption{T2 weighted, adc and high b-value images respectively}
\end{subfigure} \\
\begin{subfigure}[t]{0.46 \textwidth}
\centering
\includegraphics[height=1.0in]{PICAI_0470_t2w_gt_ax_slice14.png}
\includegraphics[height=1.0in]{PICAI_0470_t2w_500cases_nsig_ax_slice14.png}
\includegraphics[height=1.0in]{PICAI_0470_t2w_500cases_lesion_loc_ax_slice14.png}
\caption{Ground truth, lesion count and lesion location respectively}
\end{subfigure}
\caption{TODO: Pick a better inference comparison case.}\label{fig:inferenceExamples}
\end{figure}

==> tableDsc.tex <==
\begin{table}[bt!]
\centering
\begin{tabular}{c|c|c|c|}
\cline{2-4}
 & \multicolumn{3}{|c|}{Manually Labeled Cases} \\
\hline
\multicolumn{1}{|c|}{Method} & 300 & 500 & 1315 \\
\hline
\multicolumn{1}{|c|}{Supervised Learning} & 0.334 & 0.366 & 0.424 \\
\multicolumn{1}{|c|}{Lesion Count SSL} & 0.372 & 0.399 & 0.435 \\
\multicolumn{1}{|c|}{Lesion Location SSL} & 0.380 & 0.395 & 0.434 \\
\hline
\end{tabular}
\caption{DSC scores for baseline nnU-Net and nnU-Net trained with pseudo masks prepared with lesion count and lesion location.}
\label{tbl:dsc}
\end{table}



==> tableDscWithDSCTopLeft.tex <==
\begin{table}[bt!]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
DSC & \multicolumn{3}{|c|}{Manually Labeled Cases} \\
\hline
Method & 300 & 500 & 1315 \\
\hline
Supervised Learning & 0.334 & 0.366 & 0.424 \\
Lesion Count SSL & 0.372 & 0.399 & 0.435 \\
Lesion Location SSL & 0.380 & 0.395 & 0.434 \\
\hline
\end{tabular}
\caption{DSC scores for baseline nnU-Net and nnU-Net trained with pseudo masks prepared with lesion count and lesion location.}
\label{tbl:dsc}
\end{table}



==> tableDscWithDscCols.tex <==
\begin{table}[bt!]
\centering
\begin{tabular}{c|c|c|c|}
\cline{2-4}
 & \multicolumn{3}{|c|}{Manually Labeled Cases} \\
\cline{2-4}
 & 300 & 500 & 1315 \\
\hline
%\multicolumn{1}{|c|}{Method} & DSC & DSC & DSC \\
\multicolumn{1}{|c|}{Method} & \multicolumn{3}{|c|}{DSC} \\
\hline
\multicolumn{1}{|c|}{Supervised Learning} & 0.334 & 0.366 & 0.424 \\
\multicolumn{1}{|c|}{Lesion Count SSL} & 0.372 & 0.399 & 0.435 \\
\multicolumn{1}{|c|}{Lesion Location SSL} & 0.380 & 0.395 & 0.434 \\
\hline
\end{tabular}
\caption{DSC scores for baseline nnU-Net and nnU-Net trained with pseudo masks prepared with lesion count and lesion location.}
\label{tbl:dsc}
\end{table}



==> tablefROC_FPpC.tex <==
\begin{table}[t]
\centering
\begin{tabular}{c|c|c|c|}
\cline{2-4}
 & \multicolumn{3}{|c|}{Manually Labeled Cases} \\
\hline
\multicolumn{1}{|c|}{Method} & 300 & 500 & 1315 \\
\hline
\multicolumn{1}{|c|}{Supervised Learning} & 0.62 & 0.58 & 0.35 \\
\multicolumn{1}{|c|}{Count-based SSL} & 0.49 & 0.47 & 0.33 \\
\multicolumn{1}{|c|}{Location-based SSL} & 0.44 & 0.44 & 0.33 \\
\hline
\end{tabular}
\caption{The false positives per case (FPpC) at sensitivity=0.6 in the Free-response Receiver Operating Characteristic (FROC) curve on the Test set using 300, 500, or 1315 manually labeled cases combined with 1634, 1434, 619 unlabeled cases, respectively.}
\label{tbl:fppc}
\end{table}



==> tablefROC_FPpCWithFPpCTopLeft.tex <==
\begin{table}[bt!]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
 FPpC & \multicolumn{3}{|c|}{Manually Labeled Cases} \\
\hline
Method & 300 & 500 & 1315 \\
\hline
Supervised Learning & 0.62 & 0.58 & 0.35 \\
Lesion Count SSL & 0.49 & 0.47 & 0.33 \\
Lesion Location SSL & 0.44 & 0.44 & 0.33 \\
\hline
\end{tabular}
\caption{The false positives per case (FPpC) at sensitivity=0.6 in the Free-response Receiver Operating Characteristic (FROC) curve on the Test set with 300, 500, or 1315 Manually Labeled Cases.}
\label{tbl:fppc}
\end{table}


